Data Sampling on MDS-resistant 10th Generation Intel Core (Ice Lake)

Microarchitectural Data Sampling (MDS) is a set of hardware vulnerabilities in Intel CPUs that allows an attacker to leak bytes of data from memory loads and stores across various security boundaries. On affected CPUs, some of these vulnerabilities were patched via microcode updates. Additionally, Intel announced that the newest microarchitectures, namely Cascade Lake and Ice Lake, were not affected by MDS. While Cascade Lake turned out to be vulnerable to the ZombieLoad v2 MDS attack (also known as TAA), Ice Lake was not affected by this attack. In this technical report, we show a variant of MSBDS (CVE2018-12126), an MDS attack, also known as Fallout, that works on Ice Lake CPUs. This variant was automatically synthesized using Transynther, a tool to find new variants of Meltdown-type attacks. Based on the findings of Transynther, we analyze different microcodes regarding this issue, showing that only microcode versions after January 2020 prevent exploitation of the vulnerability. These results show that Transynther is a valuable tool to find new variants, and also to test for regressions possibly introduced with microcode updates.

==> Makefile <==
# NOTE: change this for every paper, it is the tag for the submission
TAG ?= SBL_CCS2019

MAIN := main
LATEXRUN_BIN ?= latexrun
LATEXDIFF_GIT_BIN ?= latexdiff-git
PDFLATEX_BIN ?= pdflatex
PDFLATEX_ARGS ?= -shell-escape
BIBTOOL_BIN ?= bibtool
CHECK_DEP ?= ""

SHELL := /bin/bash

all: graphics plots pdf

ifeq ($(shell which $(LATEXDIFF_GIT_BIN) >/dev/null 2>&1; echo $$?), 1)
$(warning Note: Please consider installing ${LATEXDIFF_GIT_BIN} to use the diff targets.)
endif

ifeq ($(shell which $(LATEXRUN_BIN) >/dev/null 2>&1; echo $$?), 1)
$(warning Note: ${LATEXRUN_BIN} missing. Installing now...)
$(shell sudo wget https://raw.githubusercontent.com/aclements/latexrun/master/latexrun -O /usr/local/bin/latexrun)
$(shell sudo chmod +x /usr/local/bin/latexrun)
endif


# plots

${MAIN}.makefile: pdf
	if [ ! -f $@ ]; then echo "all:" > $@; fi

tikz:
	mkdir -p tikz


ifeq (bib,$(firstword $(MAKECMDGOALS)))
  # use the rest as arguments for "bib"
  SEARCH_ARGS := $(wordlist 2,$(words $(MAKECMDGOALS)),$(MAKECMDGOALS))
  # ...and turn them into do-nothing targets
  $(eval $(SEARCH_ARGS):;@:)
endif

%:
	@:

FORCE_BIB := 0
force-bib: FORCE_BIB := 1
force-bib: biblio

# biblio:
# 	CHECK_DEP=${CHECK_DEP} ./bibtool.sh

# bib:
# 	CHECK_DEP=${CHECK_DEP} ./bibtool.sh search $(SEARCH_ARGS)


plots: ${MAIN}.makefile tikz
	@make \
		-f ${MAIN}.makefile

plots-rebuild: ${MAIN}.makefile tikz
	@make \
		-f ${MAIN}.makefile \
		-B

# latexrun

pdf: tikz biblio
	@${LATEXRUN_BIN} \
		-O . \
		--latex-cmd=${PDFLATEX_BIN} \
		--latex-args='${PDFLATEX_ARGS}' \
		${MAIN}.tex

clean: diff-clean
	@${LATEXRUN_BIN} \
		-O . \
		--clean-all
	@rm -rf tikz *.tar *.md5

fix-linebreaks:
	@latexindent -w -m -l .latexindent-config.yaml ${MAIN}.tex

LAST_COMMIT ?= `git rev-parse HEAD`
diff:
	@${LATEXDIFF_GIT_BIN} --force --exclude-textcmd="section,subsection,subsubsection" -r ${LAST_COMMIT} -r HEAD ${MAIN}.tex --pdf

bibtool:
	@${BIBTOOL_BIN} -i ${MAIN}.bib -o ${MAIN}.bib

